The Impact of the Social Security Reforms on Welfare: Who benefits and Who loses across Generations, Gender, and Employment Type?

We quantitatively explore the impact of social security reforms in Japan, which is facing rapid aging and the highest government debt among developed countries, using an overlapping generations model with four types of agents distinguished by gender and employment type. We find that introducing social security reforms without extending the retirement age raises the welfare of future generations, while reforms with rising copayment rates for medical and long-term care expenditures, in particular, significantly lowers the welfare of low-income groups (females and part-timers) of the current retired and working generations. In contrast, reforms reducing the pension replacement rate lead to a greater decline in the welfare of full-timers. The combination of these reforms and the extension of the retirement age is expected to improve the welfare of the current working generations by 2--9 % over the level without reforms.

==> Tab/table1_pre.tex <==
%%% 2015～18年の平均値にする。

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[hbtp]
\begin{footnotesize}
\caption{Adjusted JSNA (average from 2015 to 2019)}
\label{tab:SNA}

\begin{center}
\begin{tabular}{lcc}
\hline 
& Data  \tabularnewline
\hline 
\textbf{Total adjusted income } & \textbf{1.000}  \tabularnewline
\hline 
\textbf{Labor income } & \textbf{0.509}  \tabularnewline
~~Compensation of employees  & 0.493  \tabularnewline
~~~~Wages and salaries  & 0.418   \tabularnewline
~~~~Employers' social contributions  & 0.075   \tabularnewline
~~Households' business (70\% labor income)  & 0.016  \tabularnewline
% & \tabularnewline
\hline 
\textbf{Capital income } & \textbf{0.491}  \tabularnewline
~~Corporate profits  & 0.160  \tabularnewline
~~Households' business (30 \% labor income)  & 0.007   \tabularnewline
%~~Households operating surplus  & 0.051 \tabularnewline
~~Taxes on production and imports  & 0.082   \tabularnewline
~~Less: consumption tax  & 0.039   \tabularnewline
~~Less: subsidies  & 0.006   \tabularnewline
~~Consumption of fixed capital  & 0.235   \tabularnewline
~~Statistical discrepancy  & 0.002   \tabularnewline
% & \tabularnewline
\hline 
\textbf{Total adjusted product } & \textbf{1.000}  \tabularnewline 
\hline 
\textbf{Consumption } & \textbf{0.731}  \tabularnewline
~~Private consumption  & 0.539   \tabularnewline
~~Less: consumption tax  & 0.039   \tabularnewline
~~Government consumption  & 0.192   \tabularnewline
\hline 
\textbf{Investment } & \textbf{0.248}  \tabularnewline
~~Gross private investment  & 0.198   \tabularnewline
~~~~Corporations  & 0.160   \tabularnewline
~~~~Households and NPO  & 0.038   \tabularnewline
~~Gross government investment  & 0.050   \tabularnewline
~~Changes in inventories  & 0.002   \tabularnewline
\hline 
\textbf{Net exports } & \textbf{0.002} \tabularnewline
\hline 
\end{tabular}
\end{center}

\begin{enumerate}
\item[Notes:]
%Table \ref{tab:SNA} displays the Japanese national income and product accounts, after some of the standard adjustments that make model measurements and concepts consistent with the National Accounts of Japan (JSNA). 
The adjusted GDP is equal to the JSNA GDP after subtracting consumption tax as it is assumed to be levied on private consumption. 
Following \citet{MMP2018IMF}, we categorize income as "labor" or "capital". 
Labor income comprises 53\% of the total adjusted income, and mainly consists of compensation of employees.
Also classified into labor income is 70\% of households' mixed income (including private unincorporated enterprises). 
Meanwhile, capital income includes all other categories of income, including the remaining 30\% of households' mixed income as well as households' net operating surplus (imputed service of owner-occupied dwellings).
\end{enumerate}
\end{footnotesize}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
